Gamma Ray Burst afterglow and prompt-afterglow relations: an overview

The mechanism responsible for the afterglow emission of Gamma Ray Bursts (GRBs) and its connection to the prompt $\gamma$-ray emission is still a debated issue. Relations between intrinsic properties of the prompt or afterglow emission can help to discriminate between plausible theoretical models of GRB production. Here we present an overview of the afterglow and prompt-afterglow two parameter relations, their physical interpretations, their use as redshift estimators and as possible cosmological tools. A similar task has already been correctly achieved for Supernovae (SNe) Ia by using the peak magnitude-stretch relation, known in the literature as the Phillips relation \citep{phillips93}. The challenge today is to make GRBs, which are amongst the farthest objects ever observed, standardizable candles as the SNe Ia through well established and robust relations. Thus, the study of relations amongst the observable and physical properties of GRBs is highly relevant together with selection biases in their physical quantities. Therefore, we describe the state of the art of the existing GRB relations, their possible and debated interpretations in view of the current theoretical models and how relations are corrected for selection biases. We conclude that only after an appropriate evaluation and correction for selection effects can GRB relations be used to discriminate among the theoretical models responsible for the prompt and afterglow emission and to estimate cosmological parameters.

==> hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump


